System size and energy dependence of the near-side of high-$p_T$ triggered di-hadron correlations in STAR

Previous studies have indicated that the near-side peak of high-pT triggered di-hadron correlations can be decomposed into two parts, a jet-like correlation and the ridge. We present data from Cu+Cu and Au+Au collisions at sqrt(sNN)=62 and 200 GeV, which should allow more robust tests of models. The jet-like correlation is narrow in both azimuth and pseudorapidity and has properties similar to those expected from vacuum fragmentation. The yield of particles in the jet-like correlation are presented for both systems and at both energies and compared to the yields expected from di-hadron correlations in PYTHIA 8.1. The ridge is narrow in azimuth but broad in pseudorapidity and roughly independent of pseudorapidity within STAR's acceptance. Attempts have been made to explain the production of the ridge component as coming from recombination, momentum kicks, Glasma flux tubes, and a plasma instability. However, few models have attempted to quantitatively calculate the characteristics of the ridge. The yield in the ridge is compared for all systems and energies. The implications for measurements at the LHC are discussed in context of the data and models.

==> Commands.tex <==
\newcommand{\sNNtwohundred}{$\sqrt{s_{NN}}$ = $200$ GeV\xspace}
\newcommand{\sNNsixtytwo}{$\sqrt{s_{NN}}$ = $62$ GeV\xspace}
\newcommand{\sNN}{$\sqrt{s_{NN}}$\xspace}
\newcommand{\stdassoc}{$1.5$ GeV/c $<$ $p_T^{associated}$ $<$ $p_T^{trigger}$\xspace}
\newcommand{\stdtrig}{$3.0$ $<$ $p_T^{trigger}$ $<$ $6.0$ GeV/c\xspace}
\newcommand{\pttrig}{$p_T^{trigger}$\xspace}
\newcommand{\ptassoc}{$p_T^{associated}$\xspace}
%\newcommand{\Tref}[1]{Tab.~\ref{#1}}
\newcommand{\trigrange}[2]{#1 $< p_T^{trigger} < $ #2 \xspace}
\newcommand{\assocrange}[2]{#1 $< p_T^{associated} < $ #2\xspace}
\newcommand{\assocrangevar}[1]{#1 $< p_T^{associated} < p_T^{trigger}$\xspace}
\newcommand{\detarange}[2]{#1 $< \Delta\eta < $ #2\xspace}
%
\newcommand{\npart}{$N_{part}$\xspace}
\newcommand{\nbin}{$N_{bin}$\xspace}
\newcommand{\pT}{$p_T$\xspace}
\newcommand{\mT}{$m_T$\xspace}
\newcommand{\zT}{$z_T$\xspace}
\newcommand{\KET}{$KE_T$\xspace}
\newcommand{\Nbin}{$N_{bin}$\xspace}
\newcommand{\RAA}{$R_{AA}$\xspace}
\newcommand{\RCP}{$R_{CP}$\xspace}
\newcommand{\highpT}{high-$p_T$\xspace}
\newcommand{\jet}{\textit{Jet}\xspace}
\newcommand{\njet}{$Y_{Jet}$\xspace}
\newcommand{\njetphi}{$Y_{Jet}^{\Delta\phi}$\xspace}
\newcommand{\njeteta}{$Y_{Jet}^{\Delta\eta}$\xspace}
\newcommand{\ridge}{\textit{Ridge}\xspace}
\newcommand{\nridge}{$Y_{Ridge}$\xspace}
\newcommand{\kaon}{$K^0_S$\xspace}
\newcommand{\kaondecay}{$K^0_S \rightarrow \pi^+ \pi^-$\xspace}
\newcommand{\vzero}{$V^0$\xspace}
\newcommand{\vzeros}{$V^0$s\xspace}
\newcommand{\lam}{$\Lambda$\xspace}
\newcommand{\lamdecay}{$\Lambda \rightarrow p \pi^-$\xspace}
\newcommand{\alam}{$\bar{\Lambda}$\xspace}
\newcommand{\alamdecay}{$\bar{\Lambda} \rightarrow \bar{p} \pi^+$\xspace}
%\newcommand{\lamalam}{$\frac{\Lambda+\bar{\Lambda}}{2}$\xspace}
\newcommand{\lamalam}{$\Lambda+\bar{\Lambda}$\xspace}
\newcommand{\xibary}{$\Xi^-$\xspace}
\newcommand{\myxi}{$\Xi$\xspace}
\newcommand{\xidecay}{$\Xi^- \rightarrow \Lambda \pi^- \rightarrow p \pi^- \pi^-$\xspace}
\newcommand{\axidecay}{$\bar{\Xi}^+ \rightarrow \bar{\Lambda} \pi^+ \rightarrow \bar{p} \pi^+ \pi^+$\xspace}
\newcommand{\xidecayshort}{$\Xi^- \rightarrow \Lambda \pi^-$\xspace}
\newcommand{\axidecayshort}{$\bar{\Xi}^+ \rightarrow \bar{\Lambda} \pi^+$\xspace}
\newcommand{\axibary}{$\bar{\Xi}^+$\xspace}
\newcommand{\omegabary}{$\Omega^-$\xspace}
\newcommand{\myomega}{$\Omega$\xspace}
\newcommand{\aomegabary}{$\Omega^+$\xspace}
\newcommand{\omegadecay}{$\Omega^- \rightarrow \Lambda K^- \rightarrow p \pi^- K^-$\xspace}
\newcommand{\aomegadecay}{$\bar{\Omega}^+ \rightarrow \bar{\Lambda} K^+ \rightarrow \bar{p} \pi^+ K^+$\xspace}
\newcommand{\omegadecayshort}{$\Omega^- \rightarrow \Lambda K^-$\xspace}
\newcommand{\aomegadecayshort}{$\bar{\Omega}^+ \rightarrow \bar{\Lambda} K^+$\xspace}
\newcommand{\xiaxi}{$\frac{\Xi+\bar{\Xi}}{2}$\xspace}
\newcommand{\omegaaomega}{$\frac{\Omega+\bar{\Omega}}{2}$\xspace}
\newcommand{\pp}{$p+p$\xspace}
\newcommand{\ppbar}{$p+\bar{p}$\xspace}
\newcommand{\pA}{$p+A$\xspace}
\newcommand{\eA}{$e+A$\xspace}
\newcommand{\dA}{$d+A$\xspace}
\newcommand{\ee}{$e^{+}+e^{-}$\xspace}
\newcommand{\Cu}{$Cu+Cu$\xspace}
\newcommand{\Au}{$Au+Au$\xspace}
\newcommand{\Pb}{$Pb+Pb$\xspace}
\newcommand{\dAu}{$d+Au$\xspace}
\newcommand{\AplusA}{$A+A$\xspace}
\newcommand{\MeV}{MeV/c\xspace}
\newcommand{\GeV}{GeV/c\xspace}
\newcommand{\dphi}{$\Delta\phi$\xspace}
\newcommand{\deta}{$\Delta\eta$\xspace}
\newcommand{\vtwo}{$v_2$\xspace}
\newcommand{\nearside}{near-side\xspace}
\newcommand{\awayside}{away-side\xspace}
\newcommand{\ns}{near-side\xspace}
\newcommand{\as}{away-side\xspace}
\newcommand{\baryontomeson}{$\frac{\Lambda+\bar{\Lambda}}{2K^0_S}$\xspace}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\tref}[1]{Tab.~\ref{#1}}
%\newcommand{\Eref}[1]{Equation (\ref{#1})}
%\newcommand{\Sref}[1]{Section~\ref{#1}}
\newcommand{\Fref}[1]{Fig.~\ref{#1}}
\newcommand{\Tref}[1]{Tab.~\ref{#1}}
\newcommand{\Aref}[1]{Appendix~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}
\newcommand{\Cref}[1]{Chapter~\ref{#1}}
\newcommand{\Eref}[1]{Equation \ref{#1}}
\newcommand{\nhits}{$N_{hits}$\xspace}
\newcommand{\nhitspos}{$N_{hits}^{pos}$\xspace}
\newcommand{\nhitsneg}{$N_{hits}^{neg}$\xspace}
\newcommand{\nsigdedx}{$n_{\sigma,dE/dx}$\xspace}
\newcommand{\ngammamass}{$n_{\Gamma}$\xspace}
\newcommand{\nsigdedxpos}{$n_{\sigma,dE/dx}^{pos}$\xspace}
\newcommand{\nsigdedxneg}{$n_{\sigma,dE/dx}^{neg}$\xspace}
\newcommand{\antiproton}{$\bar{p}$\xspace}
\newcommand{\proton}{$p$\xspace}
\newcommand{\piplus}{$\pi^+$\xspace}
\newcommand{\piminus}{$\pi^-$\xspace}
\newcommand{\kplus}{$\K^+$\xspace}
\newcommand{\kminus}{$K^-$\xspace}
\newcommand{\pion}{$\pi$\xspace}
\newcommand{\kaonch}{$K$\xspace}
\newcommand{\alphas}{$\alpha_{s}$\xspace}
\newcommand{\roughly}{$\approx$\xspace}
\newcommand{\baryochemical}{$\mu_{B}$\xspace}
\newcommand{\mum}{$\mu$m\xspace}
\newcommand{\refmult}{R\xspace}
\newcommand{\jl}{jet-like\xspace}
\newcommand{\jlc}{jet-like correlation\xspace}
\newcommand{\jlcs}{jet-like correlations\xspace}
\newcommand{\jly}{jet-like yield\xspace}
\newcommand{\ry}{\ridge yield\xspace}
\newcommand{\xicut}{DCA of \vzero to PV $>$ $A$*$\sqrt{ \operatorname{DCA} \operatorname{of} \operatorname{\Omega} \operatorname{to} \operatorname{PV}}$+$B$\xspace}
\newcommand{\omegacut}{DCA of \pion to PV $>$ $C$*$\sqrt{ \operatorname{DCA} \operatorname{of} \operatorname{\Omega} \operatorname{to} \operatorname{PV}}$+$D$\xspace}
\newcommand{\py}{PYTHIA\xspace}
\newcommand{\pthat}{$\hat{p_T}$\xspace}
